Automatic Cross-Replica Sharding of Weight Update in Data-Parallel Training

In data-parallel synchronous training of deep neural networks, different devices (replicas) run the same program with different partitions of the training batch, but weight update computation is repeated on all replicas, because the weights do not have a batch dimension to partition. This can be a bottleneck for performance and scalability in typical language models with large weights, and models with small per-replica batch size which is typical in large-scale training. This paper presents an approach to automatically shard the weight update computation across replicas with efficient communication primitives and data formatting, using static analysis and transformations on the training computation graph. We show this technique achieves substantial speedups on typical image and language models on Cloud TPUs, requiring no change to model code. This technique helps close the gap between traditionally expensive (ADAM) and cheap (SGD) optimizers, as they will only take a small part of training step time and have similar peak memory usage. It helped us to achieve state-of-the-art training performance in Google's MLPerf 0.6 submission.

==> Makefile <==
MASTER = main

# Source files
SOURCES = $(wildcard *.tex)
GRAPHS = $(wildcard graphs/*.ps)
FIGURES = $(wildcard figures/*.ps)
REFS = $(wildcard *.bib)

# Non-tex dependencies
DEPS =

# Commands
# Define PREFIX for special locations
ifeq (Darwin,$(shell uname -s))
PREFIX=/usr/texbin/
LATEX=$(PREFIX)latex -output-format=dvi
PDFLATEX=$(PREFIX)latex -output-format=pdf
else
# Otherwise, assume in PATH already
PREFIX=
LATEX=$(PREFIX)latex 
PDFLATEX=$(PREFIX)pdflatex 
endif

BIBTEX=$(PREFIX)bibtex -terse -min-crossrefs=1000
DVIPS=$(PREFIX)dvips
PERL=perl

# Rsync info for LasrBibtex. Use fqdn for host.
RSYNC=rsync --rsh=ssh -v
RSYNC_HOST=cofferdam.cs.utexas.edu

# MAKEGLOSSARY=makeindex
# $(MAKEGLOSSARY) -s $*.ist -t $*.glg -o $*.gls main.glo

# Add pdf and others to list of suffixes
.SUFFIXES: .pdf .ps .dvi
.PHONY : default dvi ps pdf all force clean show

# Default phony targets
default: all
dvi : $(MASTER).dvi
ps : $(MASTER).ps
pdf : $(MASTER).pdf
all: pdf
#	-rm -f *.log *.ps *.dvi *.aux *.bbl *.blg *.tpm *.out

# Command to bibtex sources as needed. The initial conditional checks
# to see whether any bibdata files were referenced. Then,
#    1) The bibdata references are extracted and separated by "perl";
#    2) Using "xargs" each bibdata is compared against the main.bbl with
#       "test" to see if any are newer; and
#    3) If any bibdata exists and is newer or if there were any
#       undefined references, "bibtex" and "latex" are
#       executed to update the .bbl file.
# The gigantic if statement thus attempts to run bibtex only if the
# .bib sources are changed (case 1) or new references are added (case
# 2).
define bibtex-as-needed 
{ if { grep -q "bibdata" $(basename $@).aux ; } \
     && { ! { $(PERL) -ane ' if ( /bibdata\{([^}]+)\}/ ) { foreach $$bib (split(",",$$1)) { chomp($$bib); print "$$bib.bib\n" ; } }' $(basename $@).aux \
       | xargs -n 1 test $(basename $@).bbl -nt ; } \
     || { grep -qi "there were undefined references" $(basename $@).log ; } ; } ; then \
    $(BIBTEX) $(basename $@) ; \
    $(LATEX_COMMAND) $(basename $@) ; \
  fi ; }
endef

# Command to re-run latex as needed. We only want to re-run latex if
# it may help---not because there was simply an error! At present, we
# re-run to update cross-references only.
# 
define latex-as-needed
{	while grep -qi "rerun to get cross-references right" $(basename $@).log ; do \
  $(LATEX_COMMAND) $(basename $@) ; done ; }
endef

#
#  Rulez!
#
%.ps:%.dvi
	$(DVIPS) -Ppdf -G0 $< -o $@

# In this rule, we initially run latex to update the .aux file, then
# fix things up as needed.
%.dvi : LATEX_COMMAND=$(LATEX)
$(MASTER).dvi : $(SOURCES) $(GRAPHS) $(REFS) $(FIGURES) Makefile $(DEPS)
	@$(LATEX_COMMAND) $(basename $@)
	@$(bibtex-as-needed)
	@$(latex-as-needed)

# In this rule, we initially run latex to update the .aux file, then
# fix things up as needed.
%.pdf : LATEX_COMMAND=$(PDFLATEX)
$(MASTER).pdf : $(SOURCES) $(GRAPHS) $(REFS) $(FIGURES) Makefile $(DEPS)
	@$(LATEX_COMMAND) $(basename $@)
	$(bibtex-as-needed)
	@$(latex-as-needed)
	@$(LATEX_COMMAND) $(basename $@)

#main.pdf pdf: main.ps main.tpm
#	latex main
#	dvips -Ppdf -G0 main.dvi -o main.ps	
#	ps2pdf -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true main.ps

%.tpm: %.ps
	ps2pdf -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true $<
	thumbpdf --modes ps2pdf $*

clean:
#	-rm -f *.log *.ps *.dvi *.aux *.bbl *.blg *.tpm *.out *.pdf

show: $(DEFAULT)
	@case "$^" in \
   *pdf) { case "`uname -s`" in Darwin) open $(MASTER).pdf & ;; *) xpdf $(MASTER).pdf & ;; esac ; } ;; \
   *) { case "`uname -s`" in Darwin) open $(MASTER).ps & ;; *) gv $(MASTER).ps & ;; esac ; } ;; \
   esac

force: clean
	$(MAKE)

